CHARA Array Observations of the Evolved Components in Symbiotic Star Systems

The nature of the mechanisms that drive mass transfer in symbiotic stars remains an area of active research in stellar astronomy. Constraining the role that both stellar winds and Roche-lobe overflow play in this process is crucial to improving our understanding of these binaries and connecting them to important transient events such as recurrent novae and Type Ia supernovae. The high-resolution capabilities of an optical interferometer can resolve the geometric structure of the red giant in symbiotic stars and help answer this question. This work presents the results of an optical interferometric study using the Center for High Angular Resolution Astronomy (CHARA) Array for the purpose of measuring the angular diameter of and imaging the cool giant in four symbiotic and related systems. Here we report \textit{H} band observations collected with MIRC-X. Model fitting and image reconstruction are used to test for Roche-lobe-filling geometries. Near-simultaneous infrared spectroscopy taken using the NASA InfraRed Telescope Facility (IRTF) is used to determine the fundamental stellar parameters of the cool giant in each system. The parametric fits reported here favor circularly symmetric disk models over elongated geometries, while imaging suggests the presence of surface features on three of these stars. We find that the three systems with constrained orbits have inferred time-averaged filling factors below unity.

==> model_fit_results_syxb.tex <==
\begin{deluxetable*}{cccccccc}
\tablecaption{Model Fits \label{tab:modelfits}}
\tablehead{
    \colhead{Model} & \colhead{Diameter (mas)} & \colhead{$\alpha$} & \colhead{Axis-Ratio} & \colhead{Position Angle (degrees)} & \colhead{$V^2_0$} & \colhead{$\chi^2_r$} & \colhead{log(Z)}
}
\startdata
\multicolumn{8}{c}{V934 Her 2022} \\
\hline
uniform disk & $1.01^{+0.00}_{-0.00}$ & -- & -- & -- & 0.206 & 312.61 & -156.32 \\
limb darkened disk & $1.01^{+0.00}_{-0.00}$ & $0.00^{+0.00}_{-0.00}$ & -- & -- & 0.206 & 312.61 & -156.32 \\
elongated disk & $1.14^{+0.00}_{-0.00}$ & -- & $0.01^{+0.01}_{-0.00}$ & $119^{+0}_{-0}$ & 0.206 & 296.30 & -148.17 \\
\hline
\multicolumn{8}{c}{V934 Her 2022 (+T3ph)} \\
\hline
uniform disk & $1.01^{+0.00}_{-0.00}$ & -- & -- & -- & 0.206 & 190.17 & -95.09 \\
limb darkened disk & $1.01^{+0.00}_{-0.00}$ & $0.00^{+0.00}_{-0.00}$ & -- & -- & 0.206 & 190.17 & -95.10 \\
elongated disk & $1.14^{+0.00}_{-0.00}$ & -- & $0.01^{+0.01}_{-0.00}$ & $119^{+0}_{-0}$ & 0.206 & 180.26 & -90.14 \\
\hline
\multicolumn{8}{c}{V934 Her 2013} \\
\hline
uniform disk & $1.04^{+0.01}_{-0.01}$ & -- & -- & -- & 0.115 & 46.72 & -23.45 \\
limb darkened disk & $1.06^{+0.04}_{-0.02}$ & $0.16^{+0.27}_{-0.12}$ & -- & -- & 0.115 & 46.72 & -23.44 \\
elongated disk & $1.08^{+0.02}_{-0.02}$ & -- & $0.05^{+0.06}_{-0.03}$ & $7^{+4}_{-4}$ & 0.115 & 44.11 & -22.19 \\
\hline
\multicolumn{8}{c}{4U 1954+31} \\
\hline
uniform disk & $0.84^{+0.00}_{-0.00}$ & -- & -- & -- & 0.141 & 48.50 & -24.28 \\
limb darkened disk & $0.85^{+0.01}_{-0.01}$ & $0.04^{+0.07}_{-0.03}$ & -- & -- & 0.141 & 48.50 & -24.28 \\
elongated disk & $0.88^{+0.01}_{-0.01}$ & -- & $0.89^{+0.02}_{-0.01}$ & $52^{+5}_{-4}$ & 0.141 & 48.33 & -24.20 \\
\hline
\enddata
\tablecomments{Model fit results for each target based on visibility curve data. Angular diameters corrected for wavelength scale: 2022 MIRC-X data divided by 1.0054 (Gardner et al.\ 2022); 2013 MIRC data divided by 1.0014 (J.\ D.\ Monnier, priv.\ comm.\ 2024). A 2\% fractional systematic uncertainty was added in quadrature to V$^2$ errors prior to fitting. $V^2_0$ is a global transfer-function scale factor fitted prior to diameter estimation (equivalent to the \texttt{V2\_0} parameter in \textsc{pmoired}); dashes indicate epochs where the fitted scale was within 2\% of unity and no correction was applied. T3$\phi$ data excluded for 2013 epochs (see Section~\ref{sec:data}). log(Z) normalized by number of data points following \citet{Kass1995}; strong evidence threshold $|\Delta\log Z| > 5$. The visibility function for each model is given in Section~\ref{sec:models}.}
\end{deluxetable*}

